Track-To-Track Association for Fusion of Dimension-Reduced Estimates

Network-centric multitarget tracking under communication constraints is considered, where dimension-reduced track estimates are exchanged. Previous work on target tracking in this subfield has focused on fusion aspects only and derived optimal ways of reducing dimensionality based on fusion performance. In this work we propose a novel problem formalization where estimates are reduced based on association performance. The problem is analyzed theoretically and problem properties are derived. The theoretical analysis leads to an optimization strategy that can be used to partly preserve association quality when reducing the dimensionality of communicated estimates. The applicability of the suggested optimization strategy is demonstrated numerically in a multitarget scenario.

==> fig/optimization-loss-function.tex <==
\draw\optpathoption{clrlg} plot coordinates {(1.000,3.832)(2.000,4.356)(3.000,3.042)(4.000,5.115)(5.000,2.877)(6.000,5.318)(7.000,2.837)(8.000,5.370)(9.000,2.827)(10.000,5.383)(11.000,2.825)(12.000,5.386)(13.000,2.824)(14.000,5.387)(15.000,2.824)(16.000,5.387)(17.000,2.824)(18.000,5.387)(19.000,2.824)(20.000,5.387)(21.000,2.824)(22.000,5.387)(23.000,2.824)(24.000,5.387)(25.000,2.824)};
\draw\optpathoption{clrsm} plot coordinates {(1.000,3.832)(2.000,3.886)(3.000,3.941)(4.000,3.996)(5.000,4.052)(6.000,4.109)(7.000,4.166)(8.000,4.224)(9.000,4.283)(10.000,4.342)(11.000,4.402)(12.000,4.463)(13.000,4.525)(14.000,4.587)(15.000,4.650)(16.000,4.713)(17.000,4.778)(18.000,4.843)(19.000,4.909)(20.000,4.976)(21.000,5.043)(22.000,5.112)(23.000,5.181)(24.000,5.251)(25.000,5.322)};
\draw\optpathoption{clrls} plot coordinates {(1.000,3.832)(2.000,5.731)(3.000,6.456)(4.000,6.466)(5.000,6.417)(6.000,6.502)(7.000,6.422)(8.000,6.463)(9.000,6.460)(10.000,6.424)(11.000,6.497)(12.000,6.386)(13.000,6.502)(14.000,6.422)(15.000,6.462)(16.000,6.460)(17.000,6.423)(18.000,6.498)(19.000,6.386)(20.000,6.502)(21.000,6.422)(22.000,6.462)(23.000,6.460)(24.000,6.423)(25.000,6.498)};



==> fig/pareto-results-data.tex <==
\foreach \x/\y in {1.504/0.291,1.504/0.291,0.047/0.317,1.336/4.717,0.421/1.895,2.283/1.033,0.052/0.134,0.020/4.575,0.461/1.251,0.692/8.916,0.520/10.291,1.115/5.801,0.775/0.971,0.008/0.806,0.596/1.000,0.190/19.942,3.573/0.078,0.566/10.646,0.037/0.344,14.805/0.843,0.005/0.530,0.032/0.007,0.284/3.107,0.083/2.385,0.407/1.416,1.018/0.090,0.105/1.713,0.083/1.174,1.311/0.334,0.860/0.038,0.146/1.879,0.000/1.209,1.751/8.811,0.944/3.464,1.489/2.262,0.055/1.416,1.851/16.382,1.327/1.276,0.919/6.954,1.437/2.855,1.151/0.250,0.265/0.749,2.384/1.806,0.176/5.047,0.541/0.134,0.148/0.086,1.459/0.396,1.969/1.971,0.109/11.730,0.201/1.826,0.670/11.663,0.992/4.055,7.761/0.272,0.001/3.072,0.815/5.498,0.385/0.098,0.591/0.004,0.010/0.367,0.023/0.035,0.097/0.112,0.599/5.191,0.106/8.662,0.000/1.350,0.466/0.183,0.059/0.278,0.493/2.929,0.002/2.704,1.554/10.201,0.710/0.040,0.187/0.000,2.495/2.378,0.355/2.729,0.088/10.360,0.011/0.129,0.242/6.162,2.805/2.280,0.321/0.075,0.881/4.993,0.003/2.353,21.682/0.742,4.055/0.265,0.259/0.747,0.106/0.758,0.237/8.073,0.041/0.061,3.708/7.533,0.000/1.312,0.194/0.003,0.279/1.314,0.195/4.809,0.001/1.660,0.000/0.303,0.046/0.011,0.137/6.213,0.255/5.026,0.000/0.081,0.385/4.081,0.660/5.906,0.531/8.491,0.329/5.234,3.324/0.360,0.005/0.788,0.158/3.986,3.136/1.675,0.296/5.101,0.004/9.799,9.103/0.809,0.008/3.510,0.127/1.675,0.182/0.050,0.057/0.110,0.288/4.094,0.067/0.111,0.441/5.329,1.871/2.812,0.005/0.497,3.080/13.145,0.073/0.718,0.834/0.173,0.138/2.297,0.444/5.266,0.423/0.037,0.478/0.291,1.161/1.525,0.187/8.082,2.366/6.151,1.742/3.145,1.473/13.908,1.829/0.330,1.462/0.775,0.250/0.449,0.000/0.268,0.196/0.135,0.149/0.087,0.070/0.430,2.201/3.604,5.659/0.961,5.472/0.985,0.025/0.040,0.076/1.381,0.605/0.047,2.052/8.517,0.007/0.181,0.646/5.365,0.429/6.589,0.003/0.775,0.891/4.959,5.959/2.796,0.026/0.997,4.091/9.183,0.989/0.022,0.000/0.268,0.246/7.020,0.908/0.015,1.188/3.992,3.822/0.119,0.525/16.196,0.037/7.836,0.080/8.252,4.094/0.409,0.013/0.089,0.336/2.528,0.370/5.120,0.434/0.879,4.657/4.738,1.081/6.132,0.255/3.538,0.063/0.240,0.032/2.106,0.385/20.295,0.200/0.132,0.071/1.054,0.057/0.554,0.085/8.571,0.993/4.897,0.044/0.061,0.027/0.779,0.337/3.198,0.018/0.868,0.393/7.359,0.005/1.369,1.277/6.027,0.220/4.164,0.425/2.400,1.410/2.296,0.670/0.002,0.009/0.155,0.675/6.539,2.023/0.016,0.124/1.883,0.828/9.348,0.231/4.938,2.038/10.585,0.301/2.707,0.144/0.110,0.169/3.345,0.765/20.647,0.010/0.107,0.628/6.591,0.033/0.803,0.037/1.163,1.143/7.786,0.145/2.963,0.608/0.080,1.162/1.630,0.210/5.523,0.180/8.872,0.711/9.804,0.430/2.662,0.001/2.638,0.099/3.866,0.155/0.035,0.209/2.010,0.014/0.786,0.016/1.107,0.516/2.912,1.321/8.147,0.585/0.556,0.320/2.146,0.577/0.666,0.609/6.135,0.277/7.003,0.974/3.156,0.462/0.682,0.261/0.991,1.099/0.047,0.003/0.160,1.006/2.454,1.656/1.932,0.916/9.280,0.046/0.153,2.176/0.146,0.074/0.030,3.828/13.959,0.645/4.896,0.191/13.373,0.913/0.013,0.201/2.064,0.047/0.967,0.069/1.068,0.378/2.951,0.155/3.933,0.397/0.417,0.035/1.672,0.052/2.344,0.660/0.413,0.087/3.431,3.296/7.003,2.525/2.109,2.241/16.980,0.130/0.060,0.418/4.640,3.826/10.091,0.094/0.439,0.033/2.788,0.765/0.232,2.869/0.422,0.256/0.421,0.902/0.000,0.006/10.536,3.492/0.747,0.016/0.210,0.513/2.030,1.653/7.656,0.687/3.419,1.058/6.389,0.288/3.054,0.135/0.091,0.163/0.023,6.860/1.997,4.678/0.112,1.133/3.018,1.311/0.974,4.553/1.261,0.004/0.266,0.295/0.535,0.190/1.449,0.241/0.971,0.013/0.447,0.927/1.131,1.060/0.850,0.448/3.976,0.001/2.286,0.041/1.244,3.780/2.740,0.013/0.487,0.807/9.268,0.124/0.254,0.602/0.063,3.690/5.069,0.054/0.420,0.406/0.050,0.106/0.581,0.125/1.843,0.591/0.099,0.953/27.984,0.158/0.121,0.170/3.299,0.012/2.812,0.251/0.639,0.591/7.076,0.105/12.961,0.057/0.173,0.007/0.060,0.732/0.052,0.000/0.126,0.261/6.273,0.310/1.741,1.516/17.984,0.261/2.360,1.681/0.036,3.149/3.638,0.571/1.777,0.020/1.035,0.102/0.057,0.088/0.137,0.791/8.261,0.387/0.091,0.853/0.096,0.378/4.826,0.028/0.311,6.936/5.951,0.011/9.417,1.184/1.172,1.557/3.926,0.123/1.884,0.114/0.010,1.430/2.787,0.603/7.086,2.078/4.424,1.513/0.806,0.461/6.378,0.801/0.060,0.239/0.009,0.216/3.457,0.144/0.656,0.273/1.968,0.418/1.574,0.440/2.957,0.555/10.149,0.449/6.677,1.687/0.288,4.455/0.912,3.080/0.040,2.647/1.293,4.073/2.224,0.001/0.962,0.139/0.981,0.053/2.303,0.027/0.000,0.003/4.667,0.048/3.034,0.970/0.000,2.158/7.098,3.687/0.041,1.374/22.698,0.002/0.749,0.000/0.299,0.470/3.937,0.004/0.324,0.392/8.197,0.077/1.090,0.339/0.062,0.029/5.620,0.019/0.083,0.527/0.866,1.310/4.776,0.032/0.669,1.101/0.364,0.075/0.073,5.845/2.568,0.800/0.915,0.677/10.598,3.936/2.652,3.489/7.180,4.667/0.122,0.075/0.545,0.066/0.124,0.300/4.123,1.397/2.369,0.039/3.077,0.136/14.364,0.718/7.858,0.124/3.108,0.144/1.952,0.341/5.052,0.345/7.845,2.853/2.675,1.345/2.815,0.159/0.196,0.636/8.525,1.278/0.007,0.002/0.451,0.148/0.062,0.139/0.154,0.474/4.882,0.289/2.173,0.001/0.917,0.191/6.446,0.001/1.621,0.572/1.011,0.051/9.972,0.086/0.727,0.891/3.336,0.036/0.757,0.181/1.058,0.278/2.414,1.158/5.591,0.996/1.126,1.709/2.514,0.922/0.235,1.784/0.006,0.103/2.460,0.252/0.028,2.131/0.045,0.238/3.599,0.212/1.316,0.154/0.474,2.774/0.360,0.643/9.374,1.304/4.343,0.068/0.320,0.803/6.682,1.008/4.933,0.633/0.182,0.256/6.626,0.002/0.511,0.929/0.928,0.741/0.022,0.586/7.108,0.441/9.995,0.087/1.271,0.455/0.228,1.461/22.633,0.159/1.870,0.045/1.414,0.299/0.004,7.671/0.367,0.002/0.904,1.021/0.000,0.006/9.746,0.138/0.855,0.082/0.499,0.183/0.050,1.111/14.252,0.322/1.853,3.028/1.843,0.001/1.981,0.072/0.495,0.925/9.160,3.474/7.877,0.735/1.902,5.287/6.316,0.383/3.332,0.302/3.842,0.345/2.135,6.866/6.439,0.796/1.197,0.956/11.790,0.516/11.361,0.002/0.543,0.036/2.414,0.003/0.007,0.000/0.358,0.547/7.278,3.007/2.245,0.202/15.106,2.148/7.620,0.414/7.139,0.559/0.073,0.259/0.938,8.320/0.598,0.799/1.716,0.561/4.319,0.010/2.119,0.761/3.231,0.010/0.356,0.012/0.844,0.723/5.937,0.030/0.032,2.301/0.110,0.005/0.117,1.308/2.558,0.449/0.126,0.623/0.005,0.597/6.220,0.839/7.989,0.005/2.242,0.427/0.213,0.265/0.495,3.635/0.067,0.003/0.582,0.236/1.868,0.222/0.041,0.296/0.005,0.204/1.303,0.001/1.930,0.102/0.732,5.007/2.416,3.304/3.185,0.319/10.163,0.110/3.677,0.451/7.991,9.594/1.251,0.013/0.244,0.806/1.430,0.272/4.479,6.510/0.831,0.018/0.593,1.360/4.305,0.402/0.009,0.648/9.298,0.187/4.741,0.731/7.089,1.442/4.676,10.439/2.976,0.051/0.320,0.073/1.723,0.014/0.087,0.036/2.617,0.569/2.030,0.074/6.188,0.173/2.059,0.157/0.352,0.001/0.705,0.758/2.030,0.567/0.133,0.530/2.499,0.096/0.761,4.234/0.183,0.910/0.118,1.294/8.230,1.080/0.210,1.062/0.448,0.020/0.134,0.085/1.001,0.060/4.203,0.392/0.019,0.618/4.886,4.740/1.188,0.330/7.332,29.755/0.786,0.029/0.470,0.028/0.186,0.814/2.238,0.151/6.185,0.067/0.682,4.294/2.169,0.464/5.732,0.412/4.247,4.088/0.324,0.651/3.457,0.324/1.937,0.331/0.016,0.001/0.038,0.034/1.923,5.177/0.067,0.588/9.472,1.112/1.866,1.471/0.387,0.198/16.601,0.310/3.598,0.340/3.666,0.229/0.011,0.231/3.585,1.102/0.721,2.066/0.566,1.805/5.995,0.531/13.057,0.230/0.610,0.336/1.588,2.641/0.303,0.452/0.110,4.139/6.301,0.000/0.062,1.730/3.100,0.071/4.995,0.596/3.355,0.093/0.206,0.014/0.371,0.733/4.005,0.150/0.064,0.334/0.734,0.797/4.447,0.038/0.473,0.038/0.113,1.653/8.184,0.030/2.405,0.019/1.614,3.085/4.095,0.144/0.004,0.000/0.595,0.538/3.752,1.585/16.079,0.423/0.984,0.045/0.529,0.653/0.010,0.111/1.301,0.006/0.373,0.100/1.866,0.279/0.022,0.108/1.711,0.151/4.882,0.192/0.474,1.202/2.480,12.399/0.528,1.784/3.683,0.222/4.850,0.247/0.986,0.563/0.014,1.117/5.903,3.877/5.721,0.004/9.349,0.362/4.031,0.018/5.416,0.399/0.047,0.753/5.542,0.531/2.081,1.429/3.861,0.003/0.223,0.476/5.441,0.095/0.212,0.074/0.191,0.716/0.322,0.261/4.678,1.378/0.011,0.000/0.001,0.065/0.324,0.006/0.550,0.399/3.006,0.079/13.676,0.016/1.646,0.844/5.527,0.016/2.013,7.010/6.523,0.648/0.384,3.292/0.001,0.656/5.990,0.034/0.250,0.801/0.090,4.043/1.451,0.385/2.145,0.315/0.204,0.068/0.092,0.300/1.999,0.249/5.058,2.131/0.025,1.375/1.218,0.004/0.082,1.375/0.350,0.305/4.077,0.174/0.283,0.272/4.973,0.125/2.408,3.563/0.767,0.068/0.016,0.040/0.877,0.176/1.574,0.659/3.883,0.285/4.167,0.157/1.243,1.147/0.090,0.373/3.263,0.437/24.421,0.124/2.123,0.137/2.717,1.705/2.168,0.036/0.743,0.067/0.443,3.859/0.050,0.367/5.946,5.767/0.328,0.012/1.102,3.997/0.422,4.440/3.284,0.084/0.786,1.417/1.686,0.212/7.934,0.093/0.008,0.218/6.163,0.152/6.137,0.782/18.015,1.783/18.793,2.127/0.071,1.522/0.572,0.092/1.762,0.000/2.720,0.032/7.980,0.502/1.208,0.022/0.792,0.502/4.121,0.039/2.174,4.249/2.296,0.033/0.246,0.134/4.557,1.274/2.207,0.683/0.058,0.985/0.886,1.192/6.684,0.074/0.216,0.095/0.215,0.013/5.986,2.702/3.972,0.861/2.209,3.185/1.297,0.056/1.080,0.010/0.863,4.362/0.350,0.726/5.653,0.043/0.235,0.030/0.651,0.701/0.456,0.103/1.098,0.026/4.372,0.882/8.893,0.916/5.645,0.434/2.484,0.118/0.052,0.802/0.059,0.221/0.461,0.831/19.887,0.083/3.651,0.194/6.305,0.699/7.274,0.030/0.009,0.868/22.209,0.576/0.530,0.098/0.892,1.028/0.289,0.021/2.245,0.384/8.216,0.118/0.005,0.100/1.195,0.475/10.518,0.127/1.948,0.880/3.206,0.175/1.710,0.004/0.809,0.394/0.905,0.126/1.065,0.992/0.034,0.839/3.759,0.524/2.035,1.956/0.027,7.556/0.901,0.239/2.980,0.323/3.408,0.036/3.230,1.114/0.037,1.655/1.995,1.242/3.129,0.205/0.244,0.123/0.166,0.009/0.717,0.474/0.038,1.412/7.490,0.654/0.116,0.056/0.044,0.359/2.532,0.129/0.753,8.851/1.059,1.354/0.107,0.755/6.219,0.055/0.202,0.065/2.971,0.427/0.053,0.103/0.449,1.436/0.355,0.262/1.411,0.095/1.138,0.862/0.042,0.289/2.146,0.999/9.351,0.047/1.951,0.404/0.379,1.197/5.587,0.313/3.506,0.990/9.262,0.169/2.515,0.834/7.786,0.511/7.009,0.557/5.512,0.320/8.331,0.337/4.557,0.817/2.895,1.549/12.672,2.307/2.782,1.485/6.758,6.351/0.343,0.240/1.494,0.720/0.012,0.029/0.006,0.509/0.025,1.320/0.096,2.636/2.203,0.532/1.930,0.211/1.422,0.000/1.162,0.084/0.871,0.187/0.583,0.150/5.884,0.527/10.874,0.281/5.450,0.109/4.113,2.522/0.025,0.265/7.149,0.006/1.282,0.137/1.839,0.023/0.590,0.055/1.227,0.960/14.395,3.334/6.303,0.086/15.730,0.099/2.614,0.402/4.295,0.845/1.081,1.227/17.533,0.099/1.464,0.250/14.456,0.037/1.280,0.103/2.340,1.281/0.017,0.511/5.937,1.502/1.194,1.055/2.943,0.005/1.183,0.141/2.053,0.198/2.028,0.302/0.007,4.178/5.209,0.272/3.951,0.247/9.987,0.745/0.015,1.057/9.571,0.062/0.008,0.757/9.140,12.688/1.184,0.162/2.805,11.307/0.414,1.370/1.771,0.426/0.371,2.686/3.984,1.138/0.010,0.177/3.942,0.669/0.041,1.674/6.387,0.857/8.835,0.008/1.748,0.001/1.737,1.055/0.358,0.476/0.024,3.827/0.400,0.288/3.076,0.804/1.909,26.647/1.585,1.758/9.365,1.001/2.319,1.425/0.093,0.312/0.030,3.649/2.767,0.320/2.094,0.420/2.653,0.084/0.698,0.162/0.120,0.003/9.812,0.216/2.433,1.356/19.802,1.885/3.562,0.632/1.145,1.715/4.594,0.578/0.237,0.106/0.760,0.077/1.501,0.003/0.581,0.854/0.144,0.432/4.671,0.055/2.792,3.476/8.275,0.216/0.169,0.414/14.071,3.916/4.985,1.259/0.658,1.653/0.701,0.057/0.002,1.352/0.048,0.365/0.052,0.003/2.769,0.334/0.118,0.241/0.131,1.755/0.199,0.999/0.108,0.224/2.246,1.982/4.073,0.307/1.222,1.691/3.540,2.661/0.120,0.794/6.165,2.654/1.298,0.034/1.379,0.370/0.003,0.167/1.417,0.128/0.046,0.000/4.518,0.567/0.173,0.132/8.606,0.111/0.606,0.242/0.002,0.328/6.678,0.103/0.159,0.445/3.932,0.551/3.344,0.060/14.635,0.273/4.305,0.387/0.005,0.292/0.654,0.527/0.001,0.002/0.451,0.094/0.012,0.485/1.925,0.718/0.264,0.060/1.989,0.622/11.195,0.118/3.446,0.908/4.167,0.065/5.559,1.502/3.256,0.144/2.825,1.175/5.365,1.429/0.368,0.267/3.264,0.025/0.117,1.661/5.185,0.298/4.679,0.000/0.198,0.234/4.180,1.137/9.473,0.456/4.199,0.243/0.028,0.128/2.071,2.657/0.853,0.339/20.357,2.550/2.626,0.003/0.387,0.083/3.807,2.538/0.171,0.189/7.749,2.818/11.692,0.301/0.641,0.408/0.004,0.198/0.021,0.293/0.524,0.307/0.175,0.001/0.286,8.459/1.875,3.062/0.913,2.151/0.030,0.371/4.992,0.139/4.334,0.640/0.006,0.921/1.613,3.798/16.247,0.253/2.555,0.269/2.185,1.588/7.477,4.768/0.039,0.017/0.204,0.058/0.061,1.257/4.931,0.440/0.005,1.955/3.560,0.436/3.047,0.843/5.613,20.136/1.009,0.972/1.755,1.122/0.066,0.024/2.242,0.967/2.838,1.146/0.023,0.104/4.597,0.162/2.308,1.503/6.025,3.345/0.213,0.369/0.072,1.564/0.058,1.377/7.857,1.375/2.140,0.022/0.001,0.074/4.147,0.353/4.935,0.212/7.150,0.577/4.437,0.625/8.027,1.059/2.789,0.351/5.268,1.902/1.570,0.098/0.004,0.399/3.307,0.665/0.220,0.173/2.063,1.553/0.518,0.027/1.648,1.740/7.633,1.149/3.998,0.752/2.977,0.061/1.389,1.528/1.620,0.341/5.247,0.000/0.009,0.080/2.422,0.008/2.712,0.429/19.020,0.970/12.002,0.873/0.491,0.171/9.100,0.883/0.054,0.426/0.629,2.185/0.210,0.093/1.123,0.001/0.602,0.727/6.945,0.007/1.606,0.000/0.367,0.109/0.223,0.004/0.226,0.008/0.201,3.183/0.449,0.946/4.712,1.419/0.132,0.308/10.386,0.039/1.028,0.193/3.983,0.024/0.864,0.011/0.092,0.610/6.633,0.296/0.244,0.472/1.734,0.430/0.094,0.025/0.776,0.175/4.909,0.209/1.526,22.210/0.524,1.050/6.444,0.035/0.273,0.803/7.394,1.279/5.248,0.698/0.456,0.099/1.640,0.707/7.032,0.006/5.066,2.106/0.551,0.024/0.851,0.505/1.556,0.215/2.648,0.899/13.753,2.434/4.167,0.236/2.815,0.730/0.170,0.084/0.007,0.053/0.851,0.038/0.061,1.808/0.476,0.300/4.141,1.528/1.250,1.961/1.168,0.011/0.097,0.343/19.969,24.041/1.977,0.635/0.354,0.027/0.551,0.084/1.658,16.033/1.547,0.006/0.119,0.996/18.533,0.086/1.406,1.063/4.596,3.139/1.186,0.189/5.616,0.086/1.198,4.802/1.972,0.022/2.200,0.009/0.080,0.332/3.940,0.534/0.001,0.458/8.137,0.291/6.256,0.775/1.631,0.852/0.004,1.889/3.669,0.390/3.854,0.305/0.840,0.511/1.542,0.004/6.311,0.180/1.135,0.066/0.057,0.364/11.785,0.727/0.432,0.000/0.952,0.037/1.243,0.174/0.505,0.184/5.309,1.130/0.028,0.901/6.382,0.304/3.428,0.004/4.973,0.249/2.861,0.778/8.161,2.431/0.565,0.248/1.015,0.223/5.076,0.286/6.030,0.582/0.054,0.089/0.007,0.024/0.030,0.628/1.446,0.036/0.025,1.290/0.271,0.484/24.417,1.059/0.808,0.613/2.729,1.637/0.796,0.137/2.008,4.808/0.685,0.505/4.665,0.014/0.127,0.020/0.124,5.264/0.032,0.388/5.081,0.006/0.304,0.458/4.691,0.490/4.501,0.323/1.397,0.004/3.221,0.099/0.399,0.880/1.955,0.472/0.017,1.000/0.258,0.005/0.915,1.421/4.801,0.085/0.262,0.489/9.720,3.872/1.927,0.008/0.143,0.019/0.183,0.165/0.614,0.382/0.015,0.056/2.343,0.014/0.122,3.815/2.099,2.795/2.502,0.922/6.262,0.103/0.215,0.361/1.296,0.003/0.381,0.768/0.002,0.896/2.392,0.380/5.766,0.001/1.544,0.303/3.079,0.255/15.342,0.090/0.565,0.018/1.670,0.311/0.030,0.577/4.448,1.488/7.866,1.894/0.038,0.728/4.213,0.708/11.884,0.209/0.248,0.772/0.008,1.443/1.853,1.149/3.663,0.282/3.416,0.000/0.380,2.219/4.808,0.008/0.565,0.107/2.418,0.894/3.395,3.057/4.032,1.587/0.529,0.019/0.197,0.132/4.887,0.125/0.797,5.938/0.788,0.260/1.077,0.666/1.133,0.291/0.089,0.099/0.205,6.883/0.417,0.241/4.493,1.268/1.943,0.000/0.313,0.391/9.857,0.238/9.914,0.843/2.086,0.003/1.442,0.135/0.011,0.555/0.363,0.661/0.090,0.112/7.141,6.395/6.019,1.730/2.080,1.312/8.976,0.892/0.565,0.114/0.060,0.049/0.498,0.677/0.492,0.796/4.913,5.802/0.162,0.553/10.793,0.848/5.523,0.727/2.477,2.288/3.855,0.016/0.351,1.449/1.288,0.022/0.056,0.323/1.132,0.271/9.573,0.270/1.269,0.156/0.468,0.579/0.003,0.920/5.471,2.396/14.047,1.188/0.013,0.137/3.543,0.515/3.443,1.638/0.740,1.260/3.810,0.772/0.031,1.015/3.599,0.001/0.480,0.252/6.481,0.099/0.248,0.500/3.814,0.045/0.489,0.986/21.613,1.014/6.955,0.412/8.876,2.427/1.594,0.291/3.239,0.174/0.008,0.558/4.087,0.021/1.100,0.852/21.022,0.975/2.529,0.049/0.349,0.310/4.911,0.517/3.535,0.193/0.125,0.043/2.398,4.015/1.450,5.562/0.729,0.102/0.695,1.672/0.156,1.931/0.048,0.003/1.139,3.407/1.335,0.425/3.409,0.282/3.846,0.273/0.540,1.072/0.021,0.142/1.395,0.696/1.528,0.290/1.221,5.133/0.115,0.020/0.020,0.125/0.428,0.387/5.969,0.179/1.254,0.161/0.078,3.939/0.702,1.704/0.812,0.002/2.280,0.062/0.000,2.067/0.983,0.035/0.562,3.006/3.362,1.152/4.840,1.246/0.281,0.099/0.025,0.195/0.712,0.029/0.340,0.075/5.039,0.324/7.328,0.515/3.057,0.076/0.000,0.359/1.708,0.266/0.064,0.029/2.909,1.402/4.595,18.424/1.310,0.138/4.791,0.424/0.015,0.001/4.426,1.657/0.406,0.672/7.513,6.428/1.663,0.619/5.443,0.022/0.298,1.038/2.047,0.029/2.223,0.283/0.037,0.806/4.297,0.089/1.529,2.351/0.402,0.961/3.776,0.128/0.004,0.150/0.037,0.942/6.457,0.064/1.072,0.721/13.753,0.045/0.020,1.773/3.158,0.011/0.466,2.412/0.027,0.020/0.015,0.304/3.523,0.245/4.934,0.002/0.509,1.266/0.024,4.344/6.191,0.168/2.369,0.129/0.318,0.045/0.030,0.517/14.506,0.385/4.611,1.886/1.335,0.888/0.022,0.939/3.191,0.635/2.391,2.735/8.939,0.019/2.655,0.087/1.424,0.291/2.170,0.063/7.314,0.449/4.131,1.557/9.324,0.259/2.595,0.089/0.124,0.453/1.902,0.084/2.932,2.563/11.188,2.605/0.401,0.025/0.974,0.407/0.307,0.047/5.045,0.001/3.594,0.019/4.234,0.222/4.092,0.648/6.305,0.001/0.058,0.005/0.728,1.650/7.414,0.552/6.424,1.150/0.294,0.026/0.901,0.190/3.598,0.103/1.952,1.328/5.005,0.235/1.534,0.024/0.099,0.011/0.355,0.253/0.134,0.883/3.787,0.994/0.015,0.004/0.725,0.015/2.071,0.205/0.119,2.633/0.063,0.084/0.299,0.251/3.361,0.779/14.843,1.494/1.115,0.000/0.329,0.125/1.609,2.605/2.290,0.017/0.954,0.090/4.007,0.007/2.598,0.283/6.306,0.022/2.245,0.244/0.209,0.015/1.505,0.053/7.137,0.166/7.815,0.226/0.006,1.428/7.095,0.254/1.004,0.070/0.320,0.110/1.537,0.192/0.129,0.328/2.197,0.053/0.785,0.074/2.961,0.476/3.677,0.863/8.016,0.204/0.537,1.927/0.979,0.052/0.126,0.161/0.065,0.443/5.894,0.194/1.382,1.096/0.036,3.488/0.971,0.022/1.584,1.999/0.439,0.481/4.081,0.182/0.672,1.769/6.735,0.084/3.174,0.993/0.061,1.070/9.215,1.473/1.364,4.635/0.371,1.035/3.821,0.323/0.268,1.574/6.664,0.000/2.302,0.002/0.319,0.833/2.362,1.229/2.478,0.736/16.019,0.940/3.917,1.732/4.112,8.350/0.741,0.031/0.214,0.394/7.419,0.085/2.735,0.371/0.126,0.031/1.247,1.509/3.392,0.789/1.964,0.207/3.746,0.001/3.376,0.006/3.881,0.088/1.054,3.571/0.846,0.506/6.111,0.892/0.044,0.954/0.125,0.023/0.106,0.000/0.067,1.232/4.638,0.576/0.001,1.197/10.333,0.589/12.872,0.066/2.459,1.886/0.257,0.037/0.100,1.077/6.156,0.025/0.143,0.000/0.578,0.207/0.750,0.353/6.995,0.166/0.241,0.725/11.651,1.397/0.405,0.021/1.562,0.155/0.720,0.165/0.012,2.552/6.454,1.043/5.823,0.563/0.015,0.246/0.204,3.899/5.975,1.876/1.806,2.560/0.550,0.171/0.040,0.046/0.113,0.019/0.146,0.474/0.007,9.649/4.180,0.003/0.436,0.093/1.220,1.517/5.093,2.124/0.000,0.489/0.915,0.054/0.160,0.394/0.122,1.016/9.047,0.700/0.050,0.755/2.223,0.459/4.125,0.538/0.554,0.333/7.248,3.177/0.001,4.081/3.249,0.849/2.403,2.134/0.104,2.582/12.621,0.000/0.858,0.206/5.170,5.396/1.459,0.104/3.276,0.622/3.484,0.079/0.752,0.038/1.682,0.053/0.484,0.440/2.441,0.616/0.467,0.152/0.136,1.067/8.675,0.330/0.115,2.096/0.104,0.017/3.038,0.122/1.919,0.013/0.002,0.057/0.005,0.144/0.274,5.716/2.629,0.047/0.948,0.577/1.236,0.351/1.300,0.851/0.691,1.354/3.148,1.205/7.918,1.284/8.737,0.962/1.670,0.160/6.495,1.091/0.329,0.117/5.706,0.114/0.230,8.360/0.847,0.049/0.073,0.091/1.055,0.530/4.192,0.758/8.197,3.009/2.178,1.744/1.605,0.010/1.716,0.255/0.028,2.711/3.628,2.669/5.179,0.291/1.114,3.784/0.997,0.322/3.207,0.091/5.048,1.394/1.592,0.677/1.232,0.007/5.818,0.043/0.890,0.382/5.739,0.088/4.545,2.058/1.048,0.003/0.078,0.215/1.437,2.814/1.589,0.031/1.607,0.098/1.305,0.793/11.233,0.261/1.014,1.948/2.263,1.500/0.340,0.297/2.351,5.252/0.536,0.344/6.806,0.968/0.027,1.851/0.596,0.415/20.421,0.000/0.347,1.795/7.629,0.013/1.364,1.219/0.053,0.018/0.117,0.263/1.116,0.045/13.376,0.066/7.795,0.000/1.594,0.675/3.743,0.155/4.870,0.397/1.388,0.789/18.451,0.018/0.966,0.004/2.281,0.393/6.374,6.923/0.448,0.294/5.939,3.279/8.884,0.006/9.455,0.562/1.298,0.293/1.746,0.491/0.808,0.034/0.335,0.470/0.211,0.237/2.739,0.055/0.447,0.027/1.301,0.568/1.181,0.203/0.080,0.187/1.912,0.155/0.512,0.354/5.127,0.107/3.414,1.396/4.360,0.756/0.474,0.001/1.410,0.630/0.040,0.244/11.721,8.179/6.217,0.896/0.958,0.078/6.748,0.015/0.654,0.852/2.642,1.323/4.207,0.051/0.185,1.618/2.864,0.460/1.171,0.208/3.167,0.594/0.311,1.724/10.680,0.117/0.454,0.227/0.934,0.623/5.988,0.475/9.038,0.783/0.254,0.017/0.025,0.664/2.782,1.439/12.103,3.238/4.213,0.179/2.852,0.495/0.411,0.939/9.636,0.352/4.446,0.691/9.880,0.228/6.380,0.362/6.804,0.625/15.773,1.234/1.438,0.160/0.179,1.240/7.603,1.828/0.984,0.787/0.135,0.000/0.937,0.983/0.617,0.926/0.044,0.055/0.407,2.553/3.038,0.477/2.514,0.825/3.590,0.344/4.578,0.000/0.340,0.466/2.882,0.625/11.765,6.452/0.278,0.019/0.424,2.804/0.118,0.223/16.796,1.933/0.012,0.032/1.167,0.000/0.882,0.032/9.317,5.720/3.491,0.172/2.918,0.240/6.400,0.031/3.168,0.225/0.072,0.470/4.794,0.116/1.832,1.176/5.875,1.032/0.059,0.104/0.016,0.358/0.020,3.774/4.957,0.376/5.061,3.964/1.994,0.279/4.282,0.151/0.107,0.158/1.051,1.855/0.257,0.069/0.001,0.519/13.591,0.021/2.425,1.051/0.093,0.599/0.012,0.358/0.000,0.641/1.315,1.336/4.310,0.022/2.055,0.093/0.013,0.232/0.002,0.979/14.074,0.062/0.008,0.880/3.705,0.282/4.699,3.219/4.365,1.142/0.821,0.264/0.007,0.956/6.156,0.844/4.687,2.119/0.667,0.169/2.746,0.295/3.527,0.098/0.479,0.129/1.770,0.062/0.529,0.223/0.209,0.102/0.260,0.002/2.665,0.814/0.294,0.274/2.385,2.908/0.020,1.288/2.190,0.221/1.386,0.191/4.383,0.588/9.459,0.035/0.600,0.193/0.504,0.019/0.800,0.110/1.286,0.546/10.096,1.442/0.982,0.400/7.121,0.629/5.691,0.171/6.053,0.064/0.446,0.070/0.214,2.068/8.657,1.068/0.828,0.342/8.146,2.244/3.122,2.191/0.770,0.930/0.681,0.014/0.211,0.138/4.738,0.266/4.811,1.043/1.472,0.230/3.022,1.608/0.001,0.151/7.141,0.823/0.233,0.056/3.650,2.464/9.204,0.794/0.380,0.077/1.364,4.156/2.506,0.438/8.273,1.189/25.193,2.560/6.698,0.823/12.298,0.371/2.640,0.121/0.168,0.085/2.656,0.275/0.005,0.040/4.712,0.175/2.913,0.001/0.392,0.069/3.590,0.694/4.872,1.846/12.899,0.007/1.095,2.615/2.931,0.031/0.140,0.028/5.031,0.643/0.217,0.257/0.278,0.147/1.443,1.105/2.219,1.382/9.169,7.251/0.139,0.428/5.947,0.171/0.418,0.066/0.000,0.669/0.361,0.274/1.003,0.963/15.265,5.201/0.267,0.063/0.222,0.674/21.676,0.107/1.946,0.874/3.153,1.024/4.490,0.036/1.908,0.620/0.875,0.649/1.665,0.000/0.367,0.054/1.522,2.381/3.376,0.003/0.494,0.027/2.766,0.105/0.786,0.790/7.493,0.121/4.876,0.835/2.308,4.031/4.138,0.024/1.576,0.164/0.000,1.140/0.025,0.048/0.966,1.091/2.112,0.026/4.007,0.115/2.277,0.060/0.000,0.022/8.145,0.199/0.839,0.004/0.489,0.012/0.993,0.378/2.029,0.461/0.016,0.823/4.418,1.827/2.121,0.163/15.206,0.049/0.707,1.685/5.823,2.963/0.709,0.002/0.674,0.321/0.598,2.811/0.295,0.008/0.628,0.003/1.033,0.146/1.027,0.002/0.543,8.707/0.801,0.091/0.152,0.668/0.609,0.432/18.795,0.586/9.468,0.549/2.556,0.577/1.013,0.003/0.110,0.200/0.286,0.024/0.009,1.581/1.223,0.732/1.582,0.534/0.775,0.893/7.660,0.876/8.242,0.066/6.335,0.030/1.641,0.194/1.139,0.038/1.464,0.163/2.444,0.407/8.690,0.221/3.798,0.425/0.062,0.890/3.728,0.741/11.157,12.743/3.801,0.231/1.485,1.183/0.099,1.284/0.253,0.845/10.990,1.209/5.442,0.051/0.169,0.558/5.251,0.305/4.149,5.364/1.990,0.063/0.276,0.027/0.460,0.919/4.469,0.618/11.934,0.017/4.497,3.556/0.456,0.497/7.745,0.337/0.016,0.209/5.344,0.656/0.024,1.044/0.793,3.282/5.962,0.363/8.396,2.139/0.304,0.560/8.418,0.996/0.024,0.114/6.205,0.017/0.527,0.165/5.595,0.063/2.071,0.060/0.030,0.296/4.340,0.207/3.561,0.020/0.060,0.582/6.111,1.542/13.249,0.458/8.398,0.196/0.030,0.490/18.538,3.460/0.567,0.080/0.991,0.002/1.231,0.924/4.153,0.056/0.035,0.141/3.892,0.482/7.496,1.119/0.213,0.051/2.925,0.660/5.347,0.482/8.474,1.164/0.002,1.122/10.666,0.074/0.058,1.326/1.435,0.027/0.076,0.316/0.021,0.149/5.600,0.657/5.835,0.434/2.285,1.229/7.231,0.193/1.667,2.046/0.504,0.108/0.193,0.614/7.288,0.000/0.186,1.206/6.586,1.375/4.890,0.732/0.123,0.889/10.229,0.697/3.199,0.519/6.430,1.055/7.634,4.240/1.987,0.138/0.370,0.460/8.212,0.568/0.001,0.188/0.087,0.309/3.404,0.806/9.022,0.337/8.903,2.268/19.414,0.244/12.228,0.159/4.042,0.753/16.846,0.133/1.747,0.137/3.351,0.206/4.607,0.607/16.789,1.683/0.006,0.863/5.603,1.224/0.000,0.036/1.014,0.071/0.923,0.489/7.294,0.009/0.087,0.111/1.499,0.001/1.307,0.204/5.209,0.293/4.436,0.240/2.278,3.768/0.530,2.616/0.463,0.074/0.383,0.028/0.267,1.774/8.218,0.100/0.930,0.530/6.812,2.451/0.511,0.093/0.310,0.285/0.001,0.272/0.008,0.646/0.001,1.116/6.145,0.902/5.467,1.986/0.334,4.830/0.574,0.669/3.339,0.694/3.028,1.878/3.805,1.308/0.037,0.785/5.901,1.256/1.602,0.476/0.009,1.123/0.244,0.034/1.009,1.117/1.050,0.817/3.291,1.005/0.037,0.304/1.455,1.683/11.056,1.396/1.458,0.109/0.011,2.271/0.090,0.001/1.212,0.167/3.087,2.486/0.875,0.385/12.169,0.130/0.396,1.692/0.321,0.049/0.043,0.838/6.736,0.092/0.568,0.465/0.129,0.773/0.113,1.347/12.287,1.911/0.007,1.007/25.815,0.318/5.119,0.053/4.063,0.024/6.324,0.538/10.160,0.052/3.429,2.894/5.413,4.207/2.148,7.804/2.796,0.166/16.271,0.009/2.611,0.298/0.010,0.010/1.358,0.540/0.102,0.005/1.288,0.275/4.375,0.108/1.381,0.011/0.034,1.665/0.575,0.011/1.439} {\fill\pointoption(\x,\y)circle[radius=\rcircle];};

\draw\optpathoption{clrlg} plot coordinates {(3.832,11.221)(10.054,4.356)(3.042,14.417)(8.393,5.115)(2.877,15.310)(8.044,5.318)(2.837,15.539)(7.960,5.370)(2.827,15.597)(7.939,5.383)(2.825,15.611)(7.934,5.386)(2.824,15.615)(7.933,5.387)(2.824,15.616)(7.932,5.387)(2.824,15.616)(7.932,5.387)(2.824,15.616)(7.932,5.387)(2.824,15.616)(7.932,5.387)(2.824,15.616)(7.932,5.387)(2.824,15.616)};
\draw\optpathoption{clrsm} plot coordinates {(3.832,11.221)(3.886,11.053)(3.941,10.887)(3.996,10.725)(4.052,10.566)(4.109,10.410)(4.166,10.257)(4.224,10.106)(4.283,9.959)(4.342,9.814)(4.402,9.672)(4.463,9.533)(4.525,9.396)(4.587,9.262)(4.650,9.130)(4.713,9.001)(4.778,8.874)(4.843,8.749)(4.909,8.627)(4.976,8.507)(5.043,8.389)(5.112,8.274)(5.181,8.160)(5.251,8.049)(5.322,7.939)};
\draw\optpathoption{clrls} plot coordinates {(3.832,11.221)(5.731,7.366)(6.456,6.548)(6.541,6.466)(6.417,6.587)(6.502,6.503)(6.587,6.422)(6.463,6.542)(6.547,6.460)(6.424,6.580)(6.508,6.497)(6.386,6.618)(6.502,6.504)(6.587,6.422)(6.462,6.542)(6.547,6.460)(6.423,6.581)(6.508,6.498)(6.386,6.619)(6.502,6.504)(6.587,6.422)(6.462,6.542)(6.547,6.460)(6.423,6.581)(6.508,6.498)};
\draw[black,fill=black](3.832,11.221)circle[radius=\rcircle];



==> fig/results-data.tex <==
\fill\filloption{clrfus} (0.100,0.313)--(0.200,0.338)--(0.300,0.549)--(0.400,0.554)--(0.500,0.566)--(0.600,0.618)--(0.700,0.622)--(0.800,0.563)--(0.900,0.642)--(1.000,0.620)--(1.100,0.657)--(1.200,0.681)--(1.300,0.683)--(1.400,0.732)--(1.500,0.748)--(1.600,0.775)--(1.700,0.789)--(1.800,0.790)--(1.900,0.809)--(2.000,0.821)--(2.100,0.836)--(2.200,0.844)--(2.300,0.850)--(2.400,0.858)--(2.500,0.867)--(2.600,0.861)--(2.700,0.880)--(2.800,0.865)--(2.900,0.884)--(3.000,0.885)--(3.100,0.888)--(3.200,0.905)--(3.300,0.894)--(3.400,0.905)--(3.500,0.906)--(3.600,0.914)--(3.700,0.906)--(3.800,0.914)--(3.900,0.919)--(4.000,0.916)--(4.100,0.920)--(4.200,0.917)--(4.300,0.920)--(4.400,0.924)--(4.500,0.927)--(4.600,0.936)--(4.700,0.924)--(4.800,0.928)--(4.900,0.926)--(5.000,0.929)--(5.000,0.633)--(4.900,0.637)--(4.800,0.627)--(4.700,0.625)--(4.600,0.642)--(4.500,0.624)--(4.400,0.615)--(4.300,0.623)--(4.200,0.618)--(4.100,0.599)--(4.000,0.608)--(3.900,0.621)--(3.800,0.608)--(3.700,0.584)--(3.600,0.592)--(3.500,0.578)--(3.400,0.584)--(3.300,0.566)--(3.200,0.575)--(3.100,0.548)--(3.000,0.548)--(2.900,0.539)--(2.800,0.540)--(2.700,0.529)--(2.600,0.513)--(2.500,0.507)--(2.400,0.500)--(2.300,0.484)--(2.200,0.476)--(2.100,0.448)--(2.000,0.429)--(1.900,0.407)--(1.800,0.388)--(1.700,0.373)--(1.600,0.354)--(1.500,0.309)--(1.400,0.299)--(1.300,0.255)--(1.200,0.242)--(1.100,0.202)--(1.000,0.178)--(0.900,0.193)--(0.800,0.144)--(0.700,0.182)--(0.600,0.170)--(0.500,0.127)--(0.400,0.141)--(0.300,0.131)--(0.200,-0.042)--(0.100,-0.070)--cycle;
\draw\meanoption{clrfus} (0.100,0.121)--(0.200,0.148)--(0.300,0.340)--(0.400,0.348)--(0.500,0.346)--(0.600,0.394)--(0.700,0.402)--(0.800,0.354)--(0.900,0.418)--(1.000,0.399)--(1.100,0.429)--(1.200,0.461)--(1.300,0.469)--(1.400,0.515)--(1.500,0.528)--(1.600,0.565)--(1.700,0.581)--(1.800,0.589)--(1.900,0.608)--(2.000,0.625)--(2.100,0.642)--(2.200,0.660)--(2.300,0.667)--(2.400,0.679)--(2.500,0.687)--(2.600,0.687)--(2.700,0.705)--(2.800,0.702)--(2.900,0.712)--(3.000,0.716)--(3.100,0.718)--(3.200,0.740)--(3.300,0.730)--(3.400,0.745)--(3.500,0.742)--(3.600,0.753)--(3.700,0.745)--(3.800,0.761)--(3.900,0.770)--(4.000,0.762)--(4.100,0.760)--(4.200,0.768)--(4.300,0.772)--(4.400,0.770)--(4.500,0.775)--(4.600,0.789)--(4.700,0.774)--(4.800,0.777)--(4.900,0.782)--(5.000,0.781);

\fill\filloption{clrasso} (0.100,0.000)--(0.200,0.017)--(0.300,0.046)--(0.400,0.156)--(0.500,0.249)--(0.600,0.309)--(0.700,0.320)--(0.800,0.345)--(0.900,0.382)--(1.000,0.410)--(1.100,0.453)--(1.200,0.470)--(1.300,0.502)--(1.400,0.525)--(1.500,0.533)--(1.600,0.538)--(1.700,0.550)--(1.800,0.533)--(1.900,0.546)--(2.000,0.545)--(2.100,0.538)--(2.200,0.540)--(2.300,0.569)--(2.400,0.571)--(2.500,0.583)--(2.600,0.583)--(2.700,0.586)--(2.800,0.576)--(2.900,0.595)--(3.000,0.599)--(3.100,0.582)--(3.200,0.610)--(3.300,0.596)--(3.400,0.617)--(3.500,0.612)--(3.600,0.622)--(3.700,0.609)--(3.800,0.623)--(3.900,0.638)--(4.000,0.628)--(4.100,0.637)--(4.200,0.634)--(4.300,0.643)--(4.400,0.638)--(4.500,0.641)--(4.600,0.651)--(4.700,0.653)--(4.800,0.646)--(4.900,0.648)--(5.000,0.655)--(5.000,0.226)--(4.900,0.223)--(4.800,0.219)--(4.700,0.221)--(4.600,0.224)--(4.500,0.200)--(4.400,0.212)--(4.300,0.213)--(4.200,0.204)--(4.100,0.204)--(4.000,0.220)--(3.900,0.207)--(3.800,0.179)--(3.700,0.191)--(3.600,0.179)--(3.500,0.170)--(3.400,0.173)--(3.300,0.165)--(3.200,0.186)--(3.100,0.162)--(3.000,0.154)--(2.900,0.156)--(2.800,0.162)--(2.700,0.142)--(2.600,0.152)--(2.500,0.133)--(2.400,0.141)--(2.300,0.133)--(2.200,0.129)--(2.100,0.111)--(2.000,0.113)--(1.900,0.121)--(1.800,0.122)--(1.700,0.114)--(1.600,0.119)--(1.500,0.099)--(1.400,0.104)--(1.300,0.082)--(1.200,0.058)--(1.100,0.043)--(1.000,0.018)--(0.900,-0.002)--(0.800,-0.020)--(0.700,-0.027)--(0.600,-0.039)--(0.500,-0.047)--(0.400,-0.059)--(0.300,-0.032)--(0.200,-0.014)--(0.100,0.000)--cycle;
\draw\meanoption{clrasso} (0.100,0.000)--(0.200,0.001)--(0.300,0.007)--(0.400,0.048)--(0.500,0.101)--(0.600,0.135)--(0.700,0.147)--(0.800,0.162)--(0.900,0.190)--(1.000,0.214)--(1.100,0.248)--(1.200,0.264)--(1.300,0.292)--(1.400,0.314)--(1.500,0.316)--(1.600,0.329)--(1.700,0.332)--(1.800,0.328)--(1.900,0.333)--(2.000,0.329)--(2.100,0.325)--(2.200,0.335)--(2.300,0.351)--(2.400,0.356)--(2.500,0.358)--(2.600,0.367)--(2.700,0.364)--(2.800,0.369)--(2.900,0.376)--(3.000,0.376)--(3.100,0.372)--(3.200,0.398)--(3.300,0.381)--(3.400,0.395)--(3.500,0.391)--(3.600,0.401)--(3.700,0.400)--(3.800,0.401)--(3.900,0.422)--(4.000,0.424)--(4.100,0.420)--(4.200,0.419)--(4.300,0.428)--(4.400,0.425)--(4.500,0.420)--(4.600,0.438)--(4.700,0.437)--(4.800,0.433)--(4.900,0.436)--(5.000,0.441);

\fill\filloption{clrfull} (0.100,0.000)--(0.200,0.000)--(0.300,0.000)--(0.400,0.000)--(0.500,0.000)--(0.600,0.000)--(0.700,0.000)--(0.800,0.000)--(0.900,0.000)--(1.000,0.000)--(1.100,0.000)--(1.200,0.000)--(1.300,0.000)--(1.400,0.000)--(1.500,0.000)--(1.600,0.000)--(1.700,0.000)--(1.800,0.000)--(1.900,0.000)--(2.000,0.000)--(2.100,0.000)--(2.200,0.000)--(2.300,0.000)--(2.400,0.000)--(2.500,0.000)--(2.600,0.000)--(2.700,0.000)--(2.800,0.000)--(2.900,0.000)--(3.000,0.000)--(3.100,0.000)--(3.200,0.000)--(3.300,0.000)--(3.400,0.000)--(3.500,0.000)--(3.600,0.000)--(3.700,0.000)--(3.800,0.000)--(3.900,0.000)--(4.000,0.000)--(4.100,0.000)--(4.200,0.000)--(4.300,0.000)--(4.400,0.000)--(4.500,0.000)--(4.600,0.000)--(4.700,0.000)--(4.800,0.000)--(4.900,0.000)--(5.000,0.000)--(5.000,0.000)--(4.900,0.000)--(4.800,0.000)--(4.700,0.000)--(4.600,0.000)--(4.500,0.000)--(4.400,0.000)--(4.300,0.000)--(4.200,0.000)--(4.100,0.000)--(4.000,0.000)--(3.900,0.000)--(3.800,0.000)--(3.700,0.000)--(3.600,0.000)--(3.500,0.000)--(3.400,0.000)--(3.300,0.000)--(3.200,0.000)--(3.100,0.000)--(3.000,0.000)--(2.900,0.000)--(2.800,0.000)--(2.700,0.000)--(2.600,0.000)--(2.500,0.000)--(2.400,0.000)--(2.300,0.000)--(2.200,0.000)--(2.100,0.000)--(2.000,0.000)--(1.900,0.000)--(1.800,0.000)--(1.700,0.000)--(1.600,0.000)--(1.500,0.000)--(1.400,0.000)--(1.300,0.000)--(1.200,0.000)--(1.100,0.000)--(1.000,0.000)--(0.900,0.000)--(0.800,0.000)--(0.700,0.000)--(0.600,0.000)--(0.500,0.000)--(0.400,0.000)--(0.300,0.000)--(0.200,0.000)--(0.100,0.000)--cycle;
\draw\meanoption{clrfull} (0.100,0.000)--(0.200,0.000)--(0.300,0.000)--(0.400,0.000)--(0.500,0.000)--(0.600,0.000)--(0.700,0.000)--(0.800,0.000)--(0.900,0.000)--(1.000,0.000)--(1.100,0.000)--(1.200,0.000)--(1.300,0.000)--(1.400,0.000)--(1.500,0.000)--(1.600,0.000)--(1.700,0.000)--(1.800,0.000)--(1.900,0.000)--(2.000,0.000)--(2.100,0.000)--(2.200,0.000)--(2.300,0.000)--(2.400,0.000)--(2.500,0.000)--(2.600,0.000)--(2.700,0.000)--(2.800,0.000)--(2.900,0.000)--(3.000,0.000)--(3.100,0.000)--(3.200,0.000)--(3.300,0.000)--(3.400,0.000)--(3.500,0.000)--(3.600,0.000)--(3.700,0.000)--(3.800,0.000)--(3.900,0.000)--(4.000,0.000)--(4.100,0.000)--(4.200,0.000)--(4.300,0.000)--(4.400,0.000)--(4.500,0.000)--(4.600,0.000)--(4.700,0.000)--(4.800,0.000)--(4.900,0.000)--(5.000,0.000);



==> fig/scenario-data.tex <==
% --- TARGET 1 ---
\fill\targetoption(0.00,0.00)circle[radius = \rtgt];
\draw\ellipseoption{colora}(0.00,0.00)ellipse[x radius = 0.90, y radius = 0.79, rotate = 88.44];
\draw\ellipseoption{colorb}(0.00,0.00)ellipse[x radius = 0.68, y radius = 0.33, rotate = -153.19];

% --- TARGET 2 ---
\fill\targetoption(1.00,10.00)circle[radius = \rtgt];
\draw\ellipseoption{colora}(1.00,10.00)ellipse[x radius = 0.85, y radius = 0.73, rotate = 109.46];
\draw\ellipseoption{colorb}(1.00,10.00)ellipse[x radius = 0.78, y radius = 0.55, rotate = 50.43];

% --- TARGET 3 ---
\fill\targetoption(5.00,5.00)circle[radius = \rtgt];
\draw\ellipseoption{colora}(5.00,5.00)ellipse[x radius = 1.03, y radius = 0.80, rotate = -139.35];
\draw\ellipseoption{colorb}(5.00,5.00)ellipse[x radius = 1.22, y radius = 0.71, rotate = -164.54];

% --- TARGET 4 ---
\fill\targetoption(6.00,12.00)circle[radius = \rtgt];
\draw\ellipseoption{colora}(6.00,12.00)ellipse[x radius = 1.01, y radius = 0.73, rotate = 63.21];
\draw\ellipseoption{colorb}(6.00,12.00)ellipse[x radius = 0.76, y radius = 0.53, rotate = 165.28];

% --- TARGET 5 ---
\fill\targetoption(9.00,8.00)circle[radius = \rtgt];
\draw\ellipseoption{colora}(9.00,8.00)ellipse[x radius = 0.97, y radius = 0.77, rotate = 75.83];
\draw\ellipseoption{colorb}(9.00,8.00)ellipse[x radius = 0.75, y radius = 0.66, rotate = -143.25];

% --- TARGET 6 ---
\fill\targetoption(11.00,4.00)circle[radius = \rtgt];
\draw\ellipseoption{colora}(11.00,4.00)ellipse[x radius = 1.15, y radius = 0.72, rotate = 109.10];
\draw\ellipseoption{colorb}(11.00,4.00)ellipse[x radius = 1.07, y radius = 0.84, rotate = 57.17];

% --- TARGET 7 ---
\fill\targetoption(3.00,-1.00)circle[radius = \rtgt];
\draw\ellipseoption{colora}(3.00,-1.00)ellipse[x radius = 0.79, y radius = 0.66, rotate = 144.07];
\draw\ellipseoption{colorb}(3.00,-1.00)ellipse[x radius = 0.78, y radius = 0.73, rotate = 139.79];

% --- TARGET 8 ---
\fill\targetoption(8.00,-1.00)circle[radius = \rtgt];
\draw\ellipseoption{colora}(8.00,-1.00)ellipse[x radius = 0.89, y radius = 0.65, rotate = 86.83];
\draw\ellipseoption{colorb}(8.00,-1.00)ellipse[x radius = 0.83, y radius = 0.50, rotate = -162.28];

% --- TARGET 9 ---
\fill\targetoption(-2.00,8.00)circle[radius = \rtgt];
\draw\ellipseoption{colora}(-2.00,8.00)ellipse[x radius = 1.11, y radius = 0.92, rotate = 133.64];
\draw\ellipseoption{colorb}(-2.00,8.00)ellipse[x radius = 1.05, y radius = 0.62, rotate = -140.95];

% --- TARGET 10 ---
\fill\targetoption(-3.00,3.00)circle[radius = \rtgt];
\draw\ellipseoption{colora}(-3.00,3.00)ellipse[x radius = 0.96, y radius = 0.92, rotate = -169.42];
\draw\ellipseoption{colorb}(-3.00,3.00)ellipse[x radius = 0.84, y radius = 0.54, rotate = -137.49];


